Contrast Everything: A Hierarchical Contrastive Framework for Medical Time-Series

Contrastive representation learning is crucial in medical time series analysis as it alleviates dependency on labor-intensive, domain-specific, and scarce expert annotations. However, existing contrastive learning methods primarily focus on one single data level, which fails to fully exploit the intricate nature of medical time series. To address this issue, we present COMET, an innovative hierarchical framework that leverages data consistencies at all inherent levels in medical time series. Our meticulously designed model systematically captures data consistency from four potential levels: observation, sample, trial, and patient levels. By developing contrastive loss at multiple levels, we can learn effective representations that preserve comprehensive data consistency, maximizing information utilization in a self-supervised manner. We conduct experiments in the challenging patient-independent setting. We compare COMET against six baselines using three diverse datasets, which include ECG signals for myocardial infarction and EEG signals for Alzheimer's and Parkinson's diseases. The results demonstrate that COMET consistently outperforms all baselines, particularly in setup with 10% and 1% labeled data fractions across all datasets. These results underscore the significant impact of our framework in advancing contrastive representation learning techniques for medical time series. The source code is available at https://github.com/DL4mHealth/COMET.

==> 041methodnotes.tex <==
method notes here.

==> 071broader.tex <==
Our approach for self-supervised contrastive learning improves classification performance on target datasets in inter-patient medical diagnosis scenarios. Leveraging different granularities of consistency in medical time series is crucial to enable effective and accurate contrastive learning without sufficient labels. We believe our work will encourage the research community to discover universal frameworks for other practical applications based on time series representation learning. We also hope our work can attract more researchers to the more general problem of multi-granularity consistency from other related fields.

On the society level, our work, along with the line of contrastive learning, can promote more efficient use of medical time series with the lack of labels. To specific, our model has the potential to identify patterns and anomalies that may not be immediately apparent to human experts. This could lead to earlier and more accurate diagnoses, which in turn could improve patient outcomes and reduce healthcare costs. However, the practitioners need to be aware of the limitations of the model.

All datasets in this paper are publicly available and are not associated with any privacy or security concern. Furthermore, we have followed guidelines on responsible use specified by primary authors of the datasets used in the current work.


==> 072checklist.tex <==
Checklist here.

\xiang{@Han Yu, Please check 1. is a broader impact needed in 2023 neurips website? 2. If yes, draft it. 3. Please insert the Check list here. You can see an example from my TF-C paper last year. }



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{} In abstract and introduction, we claim that TF-C is a generalizable property of time series that can support pre-training, which is well-justified in Sec.~\ref{sec:problem_formulation} and experimentally demonstrated in Sec.~\ref{sec:experiments} (our model consistently performs comparatively to or above baseline methods). 
  \item Did you describe the limitations of your work?
    \answerYes{} See Section~\ref{sec:conclusion}.
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{} See Broader Impact on Page 10. 
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{} Yes, we include an anonymous link (see Abstract) that provides the source codes with all implementation details, implementation of baselines, and eight datasets. The link will be updated to an non-anonymous link after acceptance.
  \item Did you specify all the training details (e.g., data splits, hyper-parameters, how they were chosen)?
    \answerYes{} See implementation details in Sec.~\ref{sec:experiments}. See Appendix~\ref{app:baseline_implementation} for baseline architectures and hyper-parameter settings. More details can be found in the included URL.
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{} We run experiments for 5 times and report the average value with standard deviation. See Table~\ref{tab:har2Gesture}, Tables~\ref{tab:sleep2epilepsy}-\ref{app:ecg2emg}, and Table~\ref{tab:one_to_many}.
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{} See Appendix~\ref{app:baseline_implementation}.
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{} We used eight existing datasets and 6 state-of-the-art baselines in contrastive learning and pre-training for time series. We cited the creators for every exist asset we used. See Sec.~\ref{sec:experiments}.
  \item Did you mention the license of the assets?
    \answerYes{} All dataset licenses are mentioned in the Appendix~\ref{app:4scenarios}.
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{} See the anonymous link in Abstract.
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{} All data we use is freely available for download, without any requirement to re-contact the data curator.
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{} Our datasets are public, well-established, and do not contain PII or offensive content
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}
